Information Leakage from Optical Emanations

A previously unknown form of compromising emanations has been discovered. LED status indicators on data communication equipment, under certain conditions, are shown to carry a modulated optical signal that is significantly correlated with information being processed by the device. Physical access is not required; the attacker gains access to all data going through the device, including plaintext in the case of data encryption systems. Experiments show that it is possible to intercept data under realistic conditions at a considerable distance. Many different sorts of devices, including modems and Internet Protocol routers, were found to be vulnerable. A taxonomy of compromising optical emanations is developed, and design changes are described that will successfully block this kind of "Optical TEMPEST" attack.

==> Makefile <==
target = optical_tempest

all:: $(target).pdf

figures = Figure_1.eps Figure_2.eps Figure_3.eps Figure_5.eps \
	Figure_6.eps Figure_7.eps Figure_8.eps Figure_8.5.eps \
	Figure_8.75.eps Figure_9.eps Figure_10.eps

# PDFLaTeX like to create temporary files:
temporary_figures = Figure_1-eps-converted-to.pdf \
	Figure_2-eps-converted-to.pdf Figure_3-eps-converted-to.pdf \
	Figure_5-eps-converted-to.pdf Figure_6-eps-converted-to.pdf \
	Figure_7-eps-converted-to.pdf Figure_8-eps-converted-to.pdf \
	Figure_8.5-eps-converted-to.pdf Figure_8.75-eps-converted-to.pdf \
	Figure_9-eps-converted-to.pdf Figure_10-eps-converted-to.pdf \

$(target).pdf: $(target).tex $(target).bbl $(figures) Makefile
	pdflatex $(target).tex
	# bibtex $(target)
	@if (grep "Warning" $(target).blg > /dev/null ) then false; fi
	@while grep "Rerun to get cross-references right." $(target).log ; do \
		pdflatex $(target) ; \
	done

clean:
	rm -fv $(target).log $(target).aux $(target).blg \
		$(temporary_figures)

allclean: clean
	rm -fv $(target).pdf

vi:
	vi $(target).tex

bib:
	vi $(target).bib


